Electromagnetic Inverse Scattering from a Single Transmitter

Electromagnetic Inverse Scattering Problems (EISP) seek to reconstruct relative permittivity from scattered fields and are fundamental to applications like medical imaging. This inverse process is inherently ill-posed and highly nonlinear, making it particularly challenging, especially under sparse transmitter setups, e.g., with only one transmitter. While recent machine learning-based approaches have shown promising results, they often rely on time-consuming, case-specific optimization and perform poorly under sparse transmitter setups. To address these limitations, we revisit EISP from a data-driven perspective. The scarcity of transmitters leads to an insufficient amount of measured data, which fails to capture adequate physical information for stable inversion. Accordingly, we propose a fully end-to-end and data-driven framework that predicts the relative permittivity of scatterers from measured fields, leveraging data distribution priors to compensate for the incomplete information from sparse measurements. This design enables data-driven training and feed-forward prediction of relative permittivity while maintaining strong robustness to transmitter sparsity. Extensive experiments show that our method outperforms state-of-the-art approaches in reconstruction accuracy and robustness. Notably, we demonstrate, for the first time, high-quality reconstruction from a single transmitter. This work advances practical electromagnetic imaging by providing a new, cost-effective paradigm to inverse scattering. Code and models are released at https://gomenei.github.io/SingleTX-EISP/.

==> notation.tex <==
\makeatletter
\newcommand{\thickhline}{%
    \noalign {\ifnum 0=`}\fi \hrule height 1pt
    \futurelet \reserved@a \@xhline
}

\definecolor{mygray}{gray}{.95}

\newcommand{\projpage}{\href{https://gomenei.github.io/GenEISP/}{https://gomenei.github.io/GenEISP/}\xspace}

\newcommand{\misscite}{\textcolor{red}{[C]~}}
\newcommand{\missfig}{\textcolor{red}{[Fig]~}}
\newcommand{\misstable}{\textcolor{red}{[Tab]~}}
\newcommand{\missref}{\textcolor{red}{[Ref]~}}

\newcommand{\cmark}{\textcolor{green!60!black}{\ding{51}}} % green checkmark
\newcommand{\xmark}{\textcolor{red}{\ding{55}}} 

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} 
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} 
\def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\aka{a.k.a\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

% Clever references
\crefname{algorithm}{Alg.}{Algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\crefname{table}{Tab.}{Tabs.}
\Crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}
\Crefname{figure}{Figure}{Figures}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Equation}{Equations}
\crefname{appendix}{Appx.}{Appxs.}
\Crefname{appendix}{Appendix}{Appendices}


\acrodef{sota}[SOTA]{State-of-the-Art}
\acrodef{eisp}[EISP]{Electromagnetic Inverse Scattering Problems}
\acrodef{gt}[GT]{Ground Truth}
\acrodef{bp}[BP]{backpropagation}
\acrodef{roi}[ROI]{Region of Interest}
\acrodef{rrmse}[MSE]{Relative Root-Mean-Square Error}
\acrodef{circular}[Circular]{Circular-cylinder dataset}
\acrodef{mnist}[MNIST]{MNIST dataset}
\acrodef{ifdata}[IF]{Institut Fresnel’s database}
\acrodef{3dmnist}[3D MNIST]{3D MNIST dataset}
\acrodef{3dshapenet}[3D ShapeNet]{3D ShapeNet dataset}
\acrodef{mlp}[MLP]{Multilayer Perceptron}
\acrodef{mse}[MSE]{Mean Squared Error}
\acrodef{iou}[IoU]{Intersection over Union}
\acrodef{inr}[INR]{Implicit Neural Representation}

\newcommand{\fde}{FoamDielExt\xspace}
\newcommand{\fdi}{FoamDielInt\xspace}
\newcommand{\ftd}{FoamTwinDiel\xspace}
\newcommand{\tf}{Twofold SOM\xspace}
\newcommand{\tfshort}{2-fold SOM\xspace}
\newcommand{\gs}{Gs SOM\xspace}
\newcommand{\pg}{PGAN\xspace}
\newcommand{\bps}{BPS\xspace}
\newcommand{\pn}{Physics-Net\xspace}
\newcommand{\ii}{Imaging-Interiors\xspace}
\newcommand{\iishort}{Img-Interiors\xspace}

\newcommand{\Ni}{N}
\newcommand{\Nr}{N_r}

% 总的极化电流分布
\newcommand{\J}{J\xspace}
% 总的散射电场
\newcommand{\Es}{E^\text{s}\xspace}
% 总电场
\newcommand{\Etot}{E^\text{t}}
% 总的极化电流分布（离散化）
\newcommand{\Jg}{\mathbf{J}}
% 总的散射电场（离散化）
\newcommand{\Esg}{\mathbf{E}^\text{s}\xspace}
% 总电场（离散化）
\newcommand{\Etotg}{\mathbf{E}^\text{t}}
% 介电常数的分布
\newcommand{\Epsr}{\epsilon_r}
\newcommand{\Epsrg}{\boldsymbol{\epsilon}_r}
\newcommand{\avgEpsrg}{\hat{\Epsrg}}

% 极化率
\newcommand{\xig}{\boldsymbol{\xi}}
% 波数
\newcommand{\kz}{k_0}
% 坐标
\newcommand{\x}{{\bf{x}}}
\newcommand{\xp}{{\bf{x^{\prime}}}}
\newcommand{\xt}{{\bf{x}^text{t}}}
% ROI
\newcommand{\D}{\mathcal{D}}

% 单位矩阵
\newcommand{\I}{\bf{I}}
% 入射电场
\newcommand{\Einc}{{E}^\text{i}}
\newcommand{\Eincg}{\mathbf{E}^\text{i}}
% J到Es的Green函数
\newcommand{\Gs}{\mathbf{G}^\text{s}}
% J到Etot的Green函数
\newcommand{\Gd}{\mathbf{G}^\text{d}}

% transmitters 1预测的相对介电常数
\newcommand{\Epsrone}{\hat{\boldsymbol{\epsilon}_r}^{(1)}}
% loss function
\newcommand{\Lall}{\mathcal{L}}
\newcommand{\LJ}{\mathcal{L}_\text{curr}}
\newcommand{\Leps}{\mathcal{L}_\text{perm}}
\newcommand{\Lsca}{\mathcal{L}_\text{scat}}
\newcommand{\lJ}{\lambda_\text{curr}}
\newcommand{\leps}{\lambda_\text{perm}}
\newcommand{\lsca}{\lambda_\text{scat}}

% model
\newcommand{\MLP}{F_{\theta}}

% transmitter number
\newcommand{\Ntran}{N}

% 单点的J
\newcommand{\Jpoint}{\mathbf{J}_\text{i}}
% 单点的x
\newcommand{\xpoint}{\mathbf{x}_\text{i}}
